Learn to Resolve Conversational Dependency: A Consistency Training Framework for Conversational Question Answering

One of the main challenges in conversational question answering (CQA) is to resolve the conversational dependency, such as anaphora and ellipsis. However, existing approaches do not explicitly train QA models on how to resolve the dependency, and thus these models are limited in understanding human dialogues. In this paper, we propose a novel framework, ExCorD (Explicit guidance on how to resolve Conversational Dependency) to enhance the abilities of QA models in comprehending conversational context. ExCorD first generates self-contained questions that can be understood without the conversation history, then trains a QA model with the pairs of original and self-contained questions using a consistency-based regularizer. In our experiments, we demonstrate that ExCorD significantly improves the QA models' performance by up to 1.2 F1 on QuAC, and 5.2 F1 on CANARD, while addressing the limitations of the existing approaches.

==> tables/qr_quality.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l}
\toprule
\textbf{Example \# 1} \\
\textbf{Title} : Saosin \quad \textbf{Section Title} : Arrival of Cove Reber and Saosin EP (2004-2006) \\ 
\textbf{Current Question $\tilde{q}_1$} : What do we know about Cove Reber? \\
\textbf{Generated Question} $\tilde{q}_1$ : What do we know about \underline{Saosin's} Cove Reber? \\ \midrule\midrule
\textbf{Example \# 2} \\ 
\textbf{Title} : L. K. Advani \quad \textbf{Section Title} : Prime Minister candidacy \\ 
\textbf{$q_\text{1}$} : When was he in the prime minister candidacy? \\
\textbf{$a_\text{1}$} : general elections, ending on 16 May 2009. \\
\textbf{$q_\text{2}$} : Did he win his candidacy? \\
\textbf{$a_\text{2}$} : Indian National Congress and its allies won the 2009 general elections, \\
\textbf{Current Question $q_\text{3}$} : Are there any other interesting aspects about this article? \\
\textbf{Generated Question $\tilde{q}_\text{3}$} : Are there any other interesting aspects about this article \underline{besides L. K. Advani's 2009 general elections}? \\ \midrule \midrule
\textbf{Example \# 3} \\
\textbf{Title} : Anna Politkovskaya \quad \textbf{Section Title} : The murder remains unsolved, 2016  \\ 
\textbf{Current Question $q_\text{1}$} : Did they have any clues? \\
\textbf{Generated Question $\tilde{q}_1$} : Did \underline{Anna Politkovskaya} have any clues? \\ \midrule \midrule
\textbf{Example \# 4} \\ 
\textbf{Title} : Talking Heads \quad \textbf{Section Title} : 1992-2002: Post break-up and final reunion \\ 
\textbf{$q_\text{1}$} : What happened in 1992? \\
\textbf{$a_\text{1}$} : CANNOTANSWER \\
\textbf{$q_\text{2}$} : What happened after they broke up? \\
\textbf{$a_\text{2}$} : Frantz and Weymouth, who married in 1977, had been recording on the side as Tom Tom Club since 1981. \\
\textbf{$q_\text{3}$} : Did he make any albums? \\
\textbf{$a_\text{3}$} : self-titled debut album sold almost as well as Talking Heads \\
\textbf{Current Question $q_\text{4}$} : Was it successful? \\
\textbf{Generated Question $\tilde{q}_\text{4}$} : Was \underline{CANNOTANSWER's} album successful? \\
\bottomrule
\end{tabular}}
\caption{Quality check for self-contained questions that are generated by QR models.
In the first case, the QR model successfully generates the self-contained question $\tilde{q}_1$ based on limited information.
In the second case, the self-contained question $\tilde{q}_3$ is also successfully generated by referring to both the background information and the conversation history.
In the third case, the QR model fails to rewrite the current question correctly since what ``they'' indicates does not appear in the background information (investigators in this case). 
In the fourth case, the QR model replace ``it'' with ``CANNOTANSWER'' which is the symbol that means the question is unanswerable.
}
\label{table:rewrite_samples}
\end{table*}
